R$\times$R: Rapid eXploration for Reinforcement Learning via Sampling-based Reset Distributions and Imitation Pre-training

We present a method for enabling Reinforcement Learning of motor control policies for complex skills such as dexterous manipulation. We posit that a key difficulty for training such policies is the difficulty of exploring the problem state space, as the accessible and useful regions of this space form a complex structure along manifolds of the original high-dimensional state space. This work presents a method to enable and support exploration with Sampling-based Planning. We use a generally applicable non-holonomic Rapidly-exploring Random Trees algorithm and present multiple methods to use the resulting structure to bootstrap model-free Reinforcement Learning. Our method is effective at learning various challenging dexterous motor control skills of higher difficulty than previously shown. In particular, we achieve dexterous in-hand manipulation of complex objects while simultaneously securing the object without the use of passive support surfaces. These policies also transfer effectively to real robots. A number of example videos can also be found on the project website: https://sbrl.cs.columbia.edu

==> text/declarations.tex <==
\section*{Declarations}
\noindent\textbf{Author contributions}. Gagan Khandate led this research by conceptualizing the method, validating early versions, and developing the manuscript.
Tristan L. Saidi contributed policies for policies, new tasks, extensive ablations, and results on imitation pre-training and also assisted in writing the manuscript.
Siqi Shang trained policies in simulation and policies for sim-to-real transfer for the conference version of the submission.
Eric Chang trained contact detection models for our optics-based tactile sensor.
Johnson Adams assisted in maintaining the robot firmware and sim-to-real transfer.
Yang Liu contributed to early versions of the hardware.
Seth Dennis designed and fabricated the hardware used in our experiments.
Matei Theodor Ciocarlie provided excellent guidance and mentorship throughout all the stages of this research and assisted with the manuscript.
\\~\\
\noindent\textbf{Ethical statements.} Not applicable
\\~\\
\noindent\textbf{Funding information}. This work was supported in part by the Office of Naval Research grant N00014-21-1-4010 and the National Science Foundation grant CMMI-2037101.
\\~\\
\noindent\textbf{Data availability}. Not applicable
\\~\\
\noindent\textbf{Acknowledgments}.  We would like to thank all the members of the Robotic Manipulation and Mobility Lab at Columbia University for helpful discussions and feedback on early versions of the manuscript.
